Ein Fenster zur gleichzeitigen Messung der Uebertragungsfunktion eines realen Systems und des Leistungsdichtespektrums des ueberlagerten Rauschens am Systemausgang (Teil 1)

There is already a method known from the literature with which it is possible to measure both the transfer function and the noise power spectral density of the superimposed noise at the output of a disturbed, time-invariant, real system with nonlinearities in one measurement. By using a suitable window, the frequency selectivity of the measurement of the power spectral density of the superimposed noise can be noticeably improved without significantly increasing the computational complexity of the method. The unbiasedness and consistency of the measurement method with a suitable window are proven. The measurement of the power spectral density of a zero-mean, stationary process without measuring the transfer function is investigated as a special case for both real-valued and complex-valued signals. It is derived which requirements a suitable window should meet and how it can be calculated with high numerical accuracy. -- Es gibt bereits eine aus der Literatur bekannte Methode mit der es moeglich ist in einer Messung sowohl die Uebertragungsfunktion als auch das Rauschleistungsdichtespektrum des ueberlagerten Rauschens am Ausgang eines gestoerten, zeitinvarianten, realen Systems mit Nichtlinearitaeten zu messen. Durch den Einsatz eines geeigneten Fensters kann die Frequenzselektivitaet der Messung des Leistungsdichtespektrums der Stoerung deutlich verbessert werden, ohne den Aufwand der Berechnungen des Verfahrens nennenswert zu erhoehen. Die Erwartungstreue und die Konsistenz des Messverfahren mit Fensterung wird gezeigt. Die Messung des Leistungsdichtespektrums eines mittelwertfreien, stationaeren Prozesses ohne Messung der Uebertragungsfunktion wird als Sonderfall sowohl fuer reellwertige, als auch fuer komplexwertige Signale untersucht. Es wird hergeleitet, welche Forderungen ein geeignetes Fenster erfuellen sollte und wie es sich numerisch hochgenau berechnen laesst.

==> mbild1a.tex <==
\put(    270.000000000000,    176.000000000000){\makebox(0,0){\includegraphics[
width=    540.000000000000\unitlength,height=    352.000000000000\unitlength,clip]{pbild1a.pdf}}}


==> mbild1b1.tex <==
\put(    115.000000000000,     95.000000000000){\makebox(0,0){\includegraphics[
width=    190.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild1b1.pdf}}}


==> mbild1b2.tex <==
\put(    335.000000000000,     95.000000000000){\makebox(0,0){\includegraphics[
width=    190.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild1b2.pdf}}}


==> mbild3d1.tex <==
\put(    210.000000000000,    450.000000000000){\makebox(0,0){\includegraphics[
width=    420.000000000000\unitlength,height=    280.000000000000\unitlength,clip]{pbild3d1.pdf}}}


==> mbild3d2.tex <==
\put(    210.000000000000,    150.000000000000){\makebox(0,0){\includegraphics[
width=    420.000000000000\unitlength,height=    280.000000000000\unitlength,clip]{pbild3d2.pdf}}}


==> mbild3d3.tex <==
\put(    210.000000000000,    295.000000000000){\makebox(0,0){\includegraphics[
width=    420.000000000000\unitlength,height=    590.000000000000\unitlength,clip]{pbild3d3.pdf}}}


==> mbild4b.tex <==
\put(    230.000000000000,    313.000000000000){\makebox(0,0){\includegraphics[
width=    460.000000000000\unitlength,height=    626.000000000000\unitlength,clip]{pbild4b.pdf}}}


==> mbild5a.tex <==
\put(    225.000000000000,    140.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    280.000000000000\unitlength,clip]{pbild5a.pdf}}}


==> mbild5b1.tex <==
\put(    225.000000000000,    525.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5b1.pdf}}}


==> mbild5b2.tex <==
\put(    225.000000000000,    375.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5b2.pdf}}}


==> mbild5b3.tex <==
\put(    225.000000000000,    225.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5b3.pdf}}}


==> mbild5b4.tex <==
\put(    225.000000000000,     75.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5b4.pdf}}}


==> mbild5d1.tex <==
\put(    110.000000000000,    510.000000000000){\makebox(0,0){\includegraphics[
width=    220.000000000000\unitlength,height=    140.000000000000\unitlength,clip]{pbild5d1.pdf}}}


==> mbild5d10.tex <==
\put(    370.000000000000,     70.000000000000){\makebox(0,0){\includegraphics[
width=    140.000000000000\unitlength,height=    140.000000000000\unitlength,clip]{pbild5d10.pdf}}}


==> mbild5d2.tex <==
\put(    340.000000000000,    510.000000000000){\makebox(0,0){\includegraphics[
width=    220.000000000000\unitlength,height=    140.000000000000\unitlength,clip]{pbild5d2.pdf}}}


==> mbild5d3.tex <==
\put(     70.000000000000,    370.000000000000){\makebox(0,0){\includegraphics[
width=    140.000000000000\unitlength,height=    140.000000000000\unitlength,clip]{pbild5d3.pdf}}}


==> mbild5d4.tex <==
\put(    220.000000000000,    370.000000000000){\makebox(0,0){\includegraphics[
width=    140.000000000000\unitlength,height=    140.000000000000\unitlength,clip]{pbild5d4.pdf}}}


==> mbild5d5.tex <==
\put(    370.000000000000,    370.000000000000){\makebox(0,0){\includegraphics[
width=    140.000000000000\unitlength,height=    140.000000000000\unitlength,clip]{pbild5d5.pdf}}}


==> mbild5d6.tex <==
\put(    110.000000000000,    210.000000000000){\makebox(0,0){\includegraphics[
width=    220.000000000000\unitlength,height=    140.000000000000\unitlength,clip]{pbild5d6.pdf}}}


==> mbild5d7.tex <==
\put(    340.000000000000,    210.000000000000){\makebox(0,0){\includegraphics[
width=    220.000000000000\unitlength,height=    140.000000000000\unitlength,clip]{pbild5d7.pdf}}}


==> mbild5d8.tex <==
\put(     70.000000000000,     70.000000000000){\makebox(0,0){\includegraphics[
width=    140.000000000000\unitlength,height=    140.000000000000\unitlength,clip]{pbild5d8.pdf}}}


==> mbild5d9.tex <==
\put(    220.000000000000,     70.000000000000){\makebox(0,0){\includegraphics[
width=    140.000000000000\unitlength,height=    140.000000000000\unitlength,clip]{pbild5d9.pdf}}}


==> mbild5e1.tex <==
\put(    225.000000000000,    150.000000000000){\makebox(0,0){\includegraphics[
width=    400.000000000000\unitlength,height=    300.000000000000\unitlength,clip]{pbild5e1.pdf}}}


==> mbild5e2.tex <==
\put(    225.000000000000,     85.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5e2.pdf}}}


==> mbild5e6.tex <==
\put(    225.000000000000,    300.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild5e6.pdf}}}


==> mbild5e7.tex <==
\put(    225.000000000000,    180.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild5e7.pdf}}}


==> mbild5e8.tex <==
\put(    225.000000000000,     60.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild5e8.pdf}}}


==> mbild5f.tex <==
\put(    225.000000000000,    300.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    600.000000000000\unitlength,clip]{pbild5f.pdf}}}


==> mbild5g.tex <==
\put(    225.000000000000,    300.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    600.000000000000\unitlength,clip]{pbild5g.pdf}}}


==> mbild5h.tex <==
\put(    227.000000000000,    300.000000000000){\makebox(0,0){\includegraphics[
width=    454.000000000000\unitlength,height=    600.000000000000\unitlength,clip]{pbild5h.pdf}}}


==> mbild5i1.tex <==
\put(    225.000000000000,    130.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    260.000000000000\unitlength,clip]{pbild5i1.pdf}}}


==> mbild5i2.tex <==
\put(    225.000000000000,    130.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    260.000000000000\unitlength,clip]{pbild5i2.pdf}}}


==> mbild5i3.tex <==
\put(    225.000000000000,    130.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    260.000000000000\unitlength,clip]{pbild5i3.pdf}}}


==> mbild5j1.tex <==
\put(    225.000000000000,    430.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    260.000000000000\unitlength,clip]{pbild5j1.pdf}}}


==> mbild5j2.tex <==
\put(    225.000000000000,    130.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    260.000000000000\unitlength,clip]{pbild5j2.pdf}}}


==> mbild5k1.tex <==
\put(    101.000000000000,    340.000000000000){\makebox(0,0){\includegraphics[
width=    200.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild5k1.pdf}}}


==> mbild5k2.tex <==
\put(    346.000000000000,    340.000000000000){\makebox(0,0){\includegraphics[
width=    200.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild5k2.pdf}}}


==> mbild5k3.tex <==
\put(    101.000000000000,    100.000000000000){\makebox(0,0){\includegraphics[
width=    200.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild5k3.pdf}}}


==> mbild5k4.tex <==
\put(    346.000000000000,    100.000000000000){\makebox(0,0){\includegraphics[
width=    200.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild5k4.pdf}}}


==> mbild5l.tex <==
\put(    227.000000000000,    300.000000000000){\makebox(0,0){\includegraphics[
width=    454.000000000000\unitlength,height=    600.000000000000\unitlength,clip]{pbild5l.pdf}}}


==> mbild5w1.tex <==
\put(    225.000000000000,    525.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5w1.pdf}}}


==> mbild5w2.tex <==
\put(    225.000000000000,    375.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5w2.pdf}}}


==> mbild5w3.tex <==
\put(    225.000000000000,    225.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5w3.pdf}}}


==> mbild5w4.tex <==
\put(    225.000000000000,     75.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5w4.pdf}}}


==> mbild5y1.tex <==
\put(    225.000000000000,    525.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5y1.pdf}}}


==> mbild5y2.tex <==
\put(    225.000000000000,    375.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5y2.pdf}}}


==> mbild5y3.tex <==
\put(    225.000000000000,    225.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5y3.pdf}}}


==> mbild5y4.tex <==
\put(    225.000000000000,     75.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    150.000000000000\unitlength,clip]{pbild5y4.pdf}}}

